LeakyCLIP: Extracting Training Data from CLIP

Understanding the memorization and privacy leakage risks in Contrastive Language--Image Pretraining (CLIP) is critical for ensuring the security of multimodal models. Recent studies have demonstrated the feasibility of extracting sensitive training examples from diffusion models, with conditional diffusion models exhibiting a stronger tendency to memorize and leak information. In this work, we investigate data memorization and extraction risks in CLIP through the lens of CLIP inversion, a process that aims to reconstruct training images from text prompts. To this end, we introduce \textbf{LeakyCLIP}, a novel attack framework designed to achieve high-quality, semantically accurate image reconstruction from CLIP embeddings. We identify three key challenges in CLIP inversion: 1) non-robust features, 2) limited visual semantics in text embeddings, and 3) low reconstruction fidelity. To address these challenges, LeakyCLIP employs 1) adversarial fine-tuning to enhance optimization smoothness, 2) linear transformation-based embedding alignment, and 3) Stable Diffusion-based refinement to improve fidelity. Empirical results demonstrate the superiority of LeakyCLIP, achieving over 258% improvement in Structural Similarity Index Measure (SSIM) for ViT-B-16 compared to baseline methods on LAION-2B subset. Furthermore, we uncover a pervasive leakage risk, showing that training data membership can even be successfully inferred from the metrics of low-fidelity reconstructions. Our work introduces a practical method for CLIP inversion while offering novel insights into the nature and scope of privacy risks in multimodal models. The code is in the https://github.com/dongdongunique/LeakyCLIP

==> leakyclip_discussioin.tex <==
\section{AFT-Preserved Semantic Separation and Memorization Bound}

We derive a bound connecting adversarial feature tuning, the on-manifold lower-Lipschitz constant of the image encoder, and the image-space memorization metric used in LeakyCLIP-style analysis. The key idea is that AFT should reduce nuisance sensitivity while preserving semantic separation on the natural image manifold.

\subsection{Definitions}

Let the natural image manifold be denoted by

\begin{equation}
\mathcal M \subset \mathcal X .
\end{equation}

Let the original CLIP image encoder be

\begin{equation}
f_0:\mathcal X \to \mathcal Z ,
\end{equation}

and let the AFT encoder be

\begin{equation}
f_r:\mathcal X \to \mathcal Z .
\end{equation}

For a scale parameter

\begin{equation}
s>0 ,
\end{equation}

define the scale-separated on-manifold lower-Lipschitz constant as

\begin{equation}
m_{\parallel}^{(s)}(f)
=
\inf_{\substack{x,y\in\mathcal M\\x\neq y\\\|x-y\|_2\ge s}}
\frac{
\|f(x)-f(y)\|_2
}{
\|x-y\|_2
}.
\end{equation}

This quantity measures how well the encoder separates natural images at scale at least

\begin{equation}
s .
\end{equation}

Next define the nuisance-direction Lipschitz constant

\begin{equation}
L_{\perp}(f)
=
\sup_{x\in\mathcal M}
\sup_{\substack{\xi\neq 0\\ \xi\perp T_x\mathcal M}}
\frac{
\|f(x+\xi)-f(x)\|_2
}{
\|\xi\|_2
}.
\end{equation}

This measures the encoder sensitivity to off-manifold perturbations. AFT is designed to reduce this quantity.

Define the semantic-nuisance condition number

\begin{equation}
\kappa^{(s)}(f)
=
\frac{
L_{\perp}(f)
}{
m_{\parallel}^{(s)}(f)
}.
\end{equation}

A smaller value means that the encoder is less sensitive to nuisance perturbations relative to how strongly it separates natural images.

\subsection{Assumptions}

We make the following assumptions.

\paragraph{Assumption 1: Clean-feature anchoring.}

AFT does not move clean image features too far away from the original CLIP feature geometry. There exists

\begin{equation}
\tau\ge 0
\end{equation}

such that

\begin{equation}
\sup_{x\in\mathcal M}
\|f_r(x)-f_0(x)\|_2
\le
\tau .
\end{equation}

\paragraph{Assumption 2: Nuisance suppression.}

AFT reduces nuisance sensitivity by a factor

\begin{equation}
0<q_L<1 ,
\end{equation}

that is,

\begin{equation}
L_{\perp}(f_r)
\le
q_L L_{\perp}(f_0).
\end{equation}

\paragraph{Assumption 3: Approximate inversion.}

Let

\begin{equation}
x_i\in\mathcal M
\end{equation}

be a training image, and let the target feature for inversion be obtained from a nuisance-perturbed input

\begin{equation}
\widetilde u_i
=
f(x_i+\xi_i),
\end{equation}

where

\begin{equation}
\xi_i\perp T_{x_i}\mathcal M
\end{equation}

and

\begin{equation}
\|\xi_i\|_2\le \rho_i .
\end{equation}

The inversion algorithm returns

\begin{equation}
\widehat x_i\in\mathcal M .
\end{equation}

We assume the inversion approximately minimizes the feature residual on the natural image manifold:

\begin{equation}
\|f(\widehat x_i)-\widetilde u_i\|_2
\le
\alpha
\inf_{x\in\mathcal M}
\|f(x)-\widetilde u_i\|_2
+
\beta_i ,
\end{equation}

where

\begin{equation}
\alpha\ge 1
\end{equation}

measures optimization suboptimality and

\begin{equation}
\beta_i\ge 0
\end{equation}

is the residual optimization or decoder error.

\subsection{Theorem 1: AFT Preserves On-Manifold Lower-Lipschitz Geometry}

\begin{theorem}
Suppose the clean-feature anchoring assumption holds:

\begin{equation}
\sup_{x\in\mathcal M}
\|f_r(x)-f_0(x)\|_2
\le
\tau .
\end{equation}

Then the scale-separated on-manifold lower-Lipschitz constant of the AFT encoder satisfies

\begin{equation}
m_{\parallel}^{(s)}(f_r)
\ge
m_{\parallel}^{(s)}(f_0)
-
\frac{2\tau}{s}.
\end{equation}
\end{theorem}

\begin{proof}
Take any two natural images satisfying

\begin{equation}
x,y\in\mathcal M ,
\end{equation}

\begin{equation}
x\neq y ,
\end{equation}

and

\begin{equation}
\|x-y\|_2\ge s .
\end{equation}

We begin from

\begin{equation}
\|f_r(x)-f_r(y)\|_2 .
\end{equation}

Add and subtract the original encoder features:

\begin{equation}
f_r(x)-f_r(y)
=
f_0(x)-f_0(y)
+
\bigl(f_r(x)-f_0(x)\bigr)
-
\bigl(f_r(y)-f_0(y)\bigr).
\end{equation}

By the reverse triangle inequality,

\begin{equation}
\|f_r(x)-f_r(y)\|_2
\ge
\|f_0(x)-f_0(y)\|_2
-
\|f_r(x)-f_0(x)\|_2
-
\|f_r(y)-f_0(y)\|_2 .
\end{equation}

Using clean-feature anchoring,

\begin{equation}
\|f_r(x)-f_0(x)\|_2
\le
\tau
\end{equation}

and

\begin{equation}
\|f_r(y)-f_0(y)\|_2
\le
\tau .
\end{equation}

Therefore,

\begin{equation}
\|f_r(x)-f_r(y)\|_2
\ge
\|f_0(x)-f_0(y)\|_2
-
2\tau .
\end{equation}

By the definition of

\begin{equation}
m_{\parallel}^{(s)}(f_0),
\end{equation}

we have

\begin{equation}
\|f_0(x)-f_0(y)\|_2
\ge
m_{\parallel}^{(s)}(f_0)
\|x-y\|_2 .
\end{equation}

Hence,

\begin{equation}
\|f_r(x)-f_r(y)\|_2
\ge
m_{\parallel}^{(s)}(f_0)
\|x-y\|_2
-
2\tau .
\end{equation}

Since

\begin{equation}
\|x-y\|_2\ge s ,
\end{equation}

we have

\begin{equation}
2\tau
\le
\frac{2\tau}{s}
\|x-y\|_2 .
\end{equation}

Thus,

\begin{equation}
\|f_r(x)-f_r(y)\|_2
\ge
\left(
m_{\parallel}^{(s)}(f_0)
-
\frac{2\tau}{s}
\right)
\|x-y\|_2 .
\end{equation}

Dividing both sides by

\begin{equation}
\|x-y\|_2
\end{equation}

gives

\begin{equation}
\frac{
\|f_r(x)-f_r(y)\|_2
}{
\|x-y\|_2
}
\ge
m_{\parallel}^{(s)}(f_0)
-
\frac{2\tau}{s}.
\end{equation}

Taking the infimum over all pairs satisfying the scale-separated constraint gives

\begin{equation}
m_{\parallel}^{(s)}(f_r)
\ge
m_{\parallel}^{(s)}(f_0)
-
\frac{2\tau}{s}.
\end{equation}

This proves the theorem.
\end{proof}

\subsection{Corollary 1: AFT Improves the Semantic-Nuisance Condition Number}

\begin{corollary}
Assume

\begin{equation}
L_{\perp}(f_r)
\le
q_L L_{\perp}(f_0)
\end{equation}

and

\begin{equation}
\tau
\le
\frac{1-q_L}{2}
s
m_{\parallel}^{(s)}(f_0).
\end{equation}

Then

\begin{equation}
\kappa^{(s)}(f_r)
\le
\kappa^{(s)}(f_0).
\end{equation}
\end{corollary}

\begin{proof}
From Theorem 1,

\begin{equation}
m_{\parallel}^{(s)}(f_r)
\ge
m_{\parallel}^{(s)}(f_0)
-
\frac{2\tau}{s}.
\end{equation}

Using the assumed upper bound on

\begin{equation}
\tau ,
\end{equation}

we get

\begin{equation}
\frac{2\tau}{s}
\le
(1-q_L)
m_{\parallel}^{(s)}(f_0).
\end{equation}

Therefore,

\begin{equation}
m_{\parallel}^{(s)}(f_r)
\ge
m_{\parallel}^{(s)}(f_0)
-
(1-q_L)
m_{\parallel}^{(s)}(f_0).
\end{equation}

This simplifies to

\begin{equation}
m_{\parallel}^{(s)}(f_r)
\ge
q_L
m_{\parallel}^{(s)}(f_0).
\end{equation}

Now compute the semantic-nuisance condition number of the AFT encoder:

\begin{equation}
\kappa^{(s)}(f_r)
=
\frac{
L_{\perp}(f_r)
}{
m_{\parallel}^{(s)}(f_r)
}.
\end{equation}

Using nuisance suppression and the lower bound on semantic separation,

\begin{equation}
\kappa^{(s)}(f_r)
\le
\frac{
q_L L_{\perp}(f_0)
}{
q_L m_{\parallel}^{(s)}(f_0)
}.
\end{equation}

Canceling

\begin{equation}
q_L
\end{equation}

gives

\begin{equation}
\kappa^{(s)}(f_r)
\le
\frac{
L_{\perp}(f_0)
}{
m_{\parallel}^{(s)}(f_0)
}.
\end{equation}

Therefore,

\begin{equation}
\kappa^{(s)}(f_r)
\le
\kappa^{(s)}(f_0).
\end{equation}

This proves the corollary.
\end{proof}

\subsection{Theorem 2: Image-Space Reconstruction Bound}

\begin{theorem}
Let

\begin{equation}
x_i\in\mathcal M
\end{equation}

be a training image, and let

\begin{equation}
\widetilde u_i
=
f(x_i+\xi_i)
\end{equation}

be the target feature generated from a nuisance perturbation satisfying

\begin{equation}
\|\xi_i\|_2\le \rho_i .
\end{equation}

Suppose the inversion output

\begin{equation}
\widehat x_i\in\mathcal M
\end{equation}

satisfies

\begin{equation}
\|f(\widehat x_i)-\widetilde u_i\|_2
\le
\alpha
\inf_{x\in\mathcal M}
\|f(x)-\widetilde u_i\|_2
+
\beta_i .
\end{equation}

If the encoder has on-manifold lower-Lipschitz constant

\begin{equation}
m_{\parallel}^{(s)}(f)>0
\end{equation}

on the relevant inversion basin, then

\begin{equation}
\|\widehat x_i-x_i\|_2
\le
\frac{
(\alpha+1)L_{\perp}(f)\rho_i+\beta_i
}{
m_{\parallel}^{(s)}(f)
}.
\end{equation}
\end{theorem}

\begin{proof}
First define the feature error caused by nuisance perturbation:

\begin{equation}
\epsilon_i
=
\|\widetilde u_i-f(x_i)\|_2 .
\end{equation}

Since

\begin{equation}
\widetilde u_i=f(x_i+\xi_i),
\end{equation}

we have

\begin{equation}
\epsilon_i
=
\|f(x_i+\xi_i)-f(x_i)\|_2 .
\end{equation}

By the definition of nuisance sensitivity,

\begin{equation}
\|f(x_i+\xi_i)-f(x_i)\|_2
\le
L_{\perp}(f)\|\xi_i\|_2 .
\end{equation}

Since

\begin{equation}
\|\xi_i\|_2\le \rho_i ,
\end{equation}

we obtain

\begin{equation}
\epsilon_i
\le
L_{\perp}(f)\rho_i .
\end{equation}

Now use the approximate inversion assumption:

\begin{equation}
\|f(\widehat x_i)-\widetilde u_i\|_2
\le
\alpha
\inf_{x\in\mathcal M}
\|f(x)-\widetilde u_i\|_2
+
\beta_i .
\end{equation}

Because

\begin{equation}
x_i\in\mathcal M ,
\end{equation}

the infimum is no larger than the value at

\begin{equation}
x_i .
\end{equation}

Therefore,

\begin{equation}
\inf_{x\in\mathcal M}
\|f(x)-\widetilde u_i\|_2
\le
\|f(x_i)-\widetilde u_i\|_2 .
\end{equation}

By definition,

\begin{equation}
\|f(x_i)-\widetilde u_i\|_2
=
\epsilon_i .
\end{equation}

Hence,

\begin{equation}
\|f(\widehat x_i)-\widetilde u_i\|_2
\le
\alpha\epsilon_i+\beta_i .
\end{equation}

We now bound the feature distance between

\begin{equation}
\widehat x_i
\end{equation}

and

\begin{equation}
x_i .
\end{equation}

By the triangle inequality,

\begin{equation}
\|f(\widehat x_i)-f(x_i)\|_2
\le
\|f(\widehat x_i)-\widetilde u_i\|_2
+
\|\widetilde u_i-f(x_i)\|_2 .
\end{equation}

Using the two bounds above,

\begin{equation}
\|f(\widehat x_i)-f(x_i)\|_2
\le
\alpha\epsilon_i+\beta_i+\epsilon_i .
\end{equation}

Therefore,

\begin{equation}
\|f(\widehat x_i)-f(x_i)\|_2
\le
(\alpha+1)\epsilon_i+\beta_i .
\end{equation}

Using

\begin{equation}
\epsilon_i
\le
L_{\perp}(f)\rho_i ,
\end{equation}

we get

\begin{equation}
\|f(\widehat x_i)-f(x_i)\|_2
\le
(\alpha+1)L_{\perp}(f)\rho_i+\beta_i .
\end{equation}

Now apply the on-manifold lower-Lipschitz property:

\begin{equation}
\|f(\widehat x_i)-f(x_i)\|_2
\ge
m_{\parallel}^{(s)}(f)
\|\widehat x_i-x_i\|_2 .
\end{equation}

Combining the previous two inequalities gives

\begin{equation}
m_{\parallel}^{(s)}(f)
\|\widehat x_i-x_i\|_2
\le
(\alpha+1)L_{\perp}(f)\rho_i+\beta_i .
\end{equation}

Dividing by

\begin{equation}
m_{\parallel}^{(s)}(f)
\end{equation}

yields

\begin{equation}
\|\widehat x_i-x_i\|_2
\le
\frac{
(\alpha+1)L_{\perp}(f)\rho_i+\beta_i
}{
m_{\parallel}^{(s)}(f)
}.
\end{equation}

This proves the theorem.
\end{proof}

\subsection{KL Conversion}

We now convert the image-space reconstruction bound into the point-wise memorization metric.

For each sample, define the reconstruction distribution as

\begin{equation}
p_i(x)
=
\mathcal N(\widehat x_i,\sigma^2 I),
\end{equation}

and define the reference distribution centered at the training image as

\begin{equation}
q_i(x)
=
\mathcal N(x_i,\sigma^2 I).
\end{equation}

The general KL divergence between two Gaussian distributions

\begin{equation}
p=\mathcal N(\mu_p,\Sigma_p)
\end{equation}

and

\begin{equation}
q=\mathcal N(\mu_q,\Sigma_q)
\end{equation}

in dimension

\begin{equation}
d
\end{equation}

is

\begin{equation}
D_{\mathrm{KL}}(p\|q)
=
\frac{1}{2}
\left[
\operatorname{tr}(\Sigma_q^{-1}\Sigma_p)
+
(\mu_q-\mu_p)^\top
\Sigma_q^{-1}
(\mu_q-\mu_p)
-
d
+
\log
\frac{\det \Sigma_q}{\det \Sigma_p}
\right].
\end{equation}

In our case,

\begin{equation}
\mu_p=\widehat x_i ,
\end{equation}

\begin{equation}
\mu_q=x_i ,
\end{equation}

and

\begin{equation}
\Sigma_p=\Sigma_q=\sigma^2 I .
\end{equation}

Therefore,

\begin{equation}
\Sigma_q^{-1}\Sigma_p
=
(\sigma^2 I)^{-1}(\sigma^2 I)
=
I .
\end{equation}

Hence,

\begin{equation}
\operatorname{tr}(\Sigma_q^{-1}\Sigma_p)
=
\operatorname{tr}(I)
=
d .
\end{equation}

Also,

\begin{equation}
\det \Sigma_q
=
\det \Sigma_p ,
\end{equation}

so

\begin{equation}
\log
\frac{\det \Sigma_q}{\det \Sigma_p}
=
0 .
\end{equation}

The quadratic term becomes

\begin{equation}
(\mu_q-\mu_p)^\top
\Sigma_q^{-1}
(\mu_q-\mu_p)
=
(x_i-\widehat x_i)^\top
(\sigma^2 I)^{-1}
(x_i-\widehat x_i).
\end{equation}

Since

\begin{equation}
(\sigma^2 I)^{-1}
=
\frac{1}{\sigma^2}I ,
\end{equation}

we get

\begin{equation}
(x_i-\widehat x_i)^\top
(\sigma^2 I)^{-1}
(x_i-\widehat x_i)
=
\frac{1}{\sigma^2}
\|\widehat x_i-x_i\|_2^2 .
\end{equation}

Substituting these terms into the Gaussian KL formula gives

\begin{equation}
D_{\mathrm{KL}}(p_i\|q_i)
=
\frac{1}{2}
\left[
d
+
\frac{1}{\sigma^2}
\|\widehat x_i-x_i\|_2^2
-
d
+
0
\right].
\end{equation}

The two dimension terms cancel:

\begin{equation}
d-d=0 .
\end{equation}

Thus,

\begin{equation}
D_{\mathrm{KL}}(p_i\|q_i)
=
\frac{1}{2\sigma^2}
\|\widehat x_i-x_i\|_2^2 .
\end{equation}

Using Theorem 2,

\begin{equation}
\|\widehat x_i-x_i\|_2
\le
\frac{
(\alpha+1)L_{\perp}(f)\rho_i+\beta_i
}{
m_{\parallel}^{(s)}(f)
}.
\end{equation}

Squaring both sides gives

\begin{equation}
\|\widehat x_i-x_i\|_2^2
\le
\left[
\frac{
(\alpha+1)L_{\perp}(f)\rho_i+\beta_i
}{
m_{\parallel}^{(s)}(f)
}
\right]^2 .
\end{equation}

Therefore,

\begin{equation}
D_{\mathrm{KL}}(p_i\|q_i)
\le
\frac{1}{2\sigma^2}
\left[
\frac{
(\alpha+1)L_{\perp}(f)\rho_i+\beta_i
}{
m_{\parallel}^{(s)}(f)
}
\right]^2 .
\end{equation}

\subsection{Theorem 3: Image-Space Memorization Upper Bound}

\begin{theorem}
Let the sample-wise reconstruction distributions be

\begin{equation}
p_i(x)
=
\mathcal N(\widehat x_i,\sigma^2I),
\end{equation}

and let the reference distributions be

\begin{equation}
q_i(x)
=
\mathcal N(x_i,\sigma^2I).
\end{equation}

Define the sample-wise point memorization metric as

\begin{equation}
M_{\mathrm{point}}(D;p_f)
=
\frac{1}{n}
\sum_{i=1}^{n}
D_{\mathrm{KL}}(p_i\|q_i).
\end{equation}

Under the assumptions of Theorem 2,

\begin{equation}
M_{\mathrm{point}}(D;p_f)
\le
\frac{1}{2\sigma^2 n}
\sum_{i=1}^{n}
\left[
\frac{
(\alpha+1)L_{\perp}(f)\rho_i+\beta_i
}{
m_{\parallel}^{(s)}(f)
}
\right]^2 .
\end{equation}
\end{theorem}

\begin{proof}
From the KL conversion above, each sample satisfies

\begin{equation}
D_{\mathrm{KL}}(p_i\|q_i)
\le
\frac{1}{2\sigma^2}
\left[
\frac{
(\alpha+1)L_{\perp}(f)\rho_i+\beta_i
}{
m_{\parallel}^{(s)}(f)
}
\right]^2 .
\end{equation}

Averaging this inequality over all

\begin{equation}
n
\end{equation}

training samples gives

\begin{equation}
\frac{1}{n}
\sum_{i=1}^{n}
D_{\mathrm{KL}}(p_i\|q_i)
\le
\frac{1}{n}
\sum_{i=1}^{n}
\frac{1}{2\sigma^2}
\left[
\frac{
(\alpha+1)L_{\perp}(f)\rho_i+\beta_i
}{
m_{\parallel}^{(s)}(f)
}
\right]^2 .
\end{equation}

Taking the constant

\begin{equation}
\frac{1}{2\sigma^2}
\end{equation}

outside the sum yields

\begin{equation}
M_{\mathrm{point}}(D;p_f)
\le
\frac{1}{2\sigma^2 n}
\sum_{i=1}^{n}
\left[
\frac{
(\alpha+1)L_{\perp}(f)\rho_i+\beta_i
}{
m_{\parallel}^{(s)}(f)
}
\right]^2 .
\end{equation}

This proves the theorem.
\end{proof}

\subsection{Corollary 2: AFT Memorization Bound}

Apply Theorem 3 to the AFT encoder

\begin{equation}
f_r .
\end{equation}

Using

\begin{equation}
L_{\perp}(f_r)
\le
q_L L_{\perp}(f_0)
\end{equation}

and

\begin{equation}
m_{\parallel}^{(s)}(f_r)
\ge
m_{\parallel}^{(s)}(f_0)
-
\frac{2\tau}{s},
\end{equation}

we obtain

\begin{equation}
M_{\mathrm{point}}(D;p_{f_r})
\le
\frac{1}{2\sigma^2 n}
\sum_{i=1}^{n}
\left[
\frac{
(\alpha_r+1)q_L L_{\perp}(f_0)\rho_i+\beta_{r,i}
}{
m_{\parallel}^{(s)}(f_0)-\frac{2\tau}{s}
}
\right]^2 .
\end{equation}

This bound is meaningful whenever

\begin{equation}
m_{\parallel}^{(s)}(f_0)-\frac{2\tau}{s}
>
0 .
\end{equation}

Equivalently,

\begin{equation}
\tau
<
\frac{s}{2}
m_{\parallel}^{(s)}(f_0).
\end{equation}

In the clean special case where

\begin{equation}
\beta_{r,i}=0
\end{equation}

for all samples, the bound becomes

\begin{equation}
M_{\mathrm{point}}(D;p_{f_r})
\le
\frac{
(\alpha_r+1)^2 q_L^2 L_{\perp}(f_0)^2
}{
2\sigma^2
\left(
m_{\parallel}^{(s)}(f_0)-\frac{2\tau}{s}
\right)^2
}
\cdot
\frac{1}{n}
\sum_{i=1}^{n}
\rho_i^2 .
\end{equation}

\subsection{Corollary 3: Sufficient Condition for AFT to Tighten the Memorization Upper Bound}

For the original encoder, Theorem 3 gives

\begin{equation}
M_{\mathrm{point}}(D;p_{f_0})
\le
\frac{1}{2\sigma^2 n}
\sum_{i=1}^{n}
\left[
\frac{
(\alpha_0+1)L_{\perp}(f_0)\rho_i+\beta_{0,i}
}{
m_{\parallel}^{(s)}(f_0)
}
\right]^2 .
\end{equation}

For the AFT encoder, Corollary 2 gives

\begin{equation}
M_{\mathrm{point}}(D;p_{f_r})
\le
\frac{1}{2\sigma^2 n}
\sum_{i=1}^{n}
\left[
\frac{
(\alpha_r+1)q_L L_{\perp}(f_0)\rho_i+\beta_{r,i}
}{
m_{\parallel}^{(s)}(f_0)-\frac{2\tau}{s}
}
\right]^2 .
\end{equation}

A sufficient condition for the AFT upper bound to be no larger than the original upper bound is that, for every sample,

\begin{equation}
\frac{
(\alpha_r+1)q_L L_{\perp}(f_0)\rho_i+\beta_{r,i}
}{
m_{\parallel}^{(s)}(f_0)-\frac{2\tau}{s}
}
\le
\frac{
(\alpha_0+1)L_{\perp}(f_0)\rho_i+\beta_{0,i}
}{
m_{\parallel}^{(s)}(f_0)
}.
\end{equation}

In the clean special case where

\begin{equation}
\alpha_r\le \alpha_0
\end{equation}

and

\begin{equation}
\beta_{r,i}\le \beta_{0,i}=0 ,
\end{equation}

it is sufficient that

\begin{equation}
\frac{
q_L
}{
m_{\parallel}^{(s)}(f_0)-\frac{2\tau}{s}
}
\le
\frac{
1
}{
m_{\parallel}^{(s)}(f_0)
}.
\end{equation}

This is equivalent to

\begin{equation}
q_L m_{\parallel}^{(s)}(f_0)
\le
m_{\parallel}^{(s)}(f_0)-\frac{2\tau}{s}.
\end{equation}

Rearranging gives

\begin{equation}
\frac{2\tau}{s}
\le
(1-q_L)
m_{\parallel}^{(s)}(f_0).
\end{equation}

Equivalently,

\begin{equation}
\tau
\le
\frac{1-q_L}{2}
s
m_{\parallel}^{(s)}(f_0).
\end{equation}

Therefore, if the clean-feature drift caused by AFT is not too large compared with its reduction of nuisance sensitivity, then AFT tightens the derived image-space memorization upper bound.

\subsection{Interpretation}

The derived result shows that AFT affects the memorization bound through two competing effects.

First, AFT reduces nuisance sensitivity:

\begin{equation}
L_{\perp}(f_r)
\le
q_L L_{\perp}(f_0).
\end{equation}

Second, AFT may distort the original semantic feature geometry. Clean-feature anchoring controls this distortion:

\begin{equation}
m_{\parallel}^{(s)}(f_r)
\ge
m_{\parallel}^{(s)}(f_0)
-
\frac{2\tau}{s}.
\end{equation}

Thus, AFT improves the relevant geometry when the reduction in nuisance sensitivity is larger than the loss of semantic separation:

\begin{equation}
\frac{
L_{\perp}(f_r)
}{
m_{\parallel}^{(s)}(f_r)
}
\le
\frac{
L_{\perp}(f_0)
}{
m_{\parallel}^{(s)}(f_0)
}.
\end{equation}

Under this condition, the image-space memorization upper bound becomes tighter:

\begin{equation}
M_{\mathrm{point}}(D;p_{f_r})
\le_{\mathrm{ub}}
M_{\mathrm{point}}(D;p_{f_0}).
\end{equation}

This means that AFT does not need to directly increase the lower-Lipschitz constant. Instead, it is enough that AFT suppresses off-manifold feature variation while keeping the original CLIP semantic geometry approximately anchored.
